Adaptive Non-Parametric Regression With the $K$-NN Fused Lasso

The fused lasso, also known as total-variation denoising, is a locally-adaptive function estimator over a regular grid of design points. In this paper, we extend the fused lasso to settings in which the points do not occur on a regular grid, leading to an approach for non-parametric regression. This approach, which we call the $K$-nearest neighbors ($K$-NN) fused lasso, involves (i) computing the $K$-NN graph of the design points; and (ii) performing the fused lasso over this $K$-NN graph. We show that this procedure has a number of theoretical advantages over competing approaches: specifically, it inherits local adaptivity from its connection to the fused lasso, and it inherits manifold adaptivity from its connection to the $K$-NN approach. We show that excellent results are obtained in a simulation study and on an application to flu data. For completeness, we also study an estimator that makes use of an $\epsilon$-graph rather than a $K$-NN graph, and contrast this with the $K$-NN fused lasso.

==> discussion.tex <==
\section{Conclusion}\label{sec:discussion}
%\textcolor{red}{If you submit to Biometrika then you should delete this section (see BMKA style guide).
%If submitting to another journal then keep it in.}


In this paper, we introduced a two-stage non-parametric regression estimator, by (i) constructing a nearest-neighbors graph over the observations; and (ii) performing the fused lasso over the graph. 
We have shown that when the $K$-NN or $\epsilon$-NN graph is used, the resulting procedure is locally adaptive; furthermore, when the $K$-NN graph is used, the procedure is manifold adaptive. 
Our theoretical results are bolstered by findings on simulated data and on a flu data set. 



